Conditional probability density functional theory

We present conditional probability (CP) density functional theory (DFT) as a formally exact theory. In essence, CP-DFT determines the ground-state energy of a system by finding the CP density from a series of independent Kohn-Sham (KS) DFT calculations. By directly calculating CP densities, we bypass the need for an approximate XC energy functional. In this work we discuss and derive several key properties of the CP density and corresponding CP-KS potential. Illustrative examples are used throughout to help guide the reader through the various concepts and theory presented. We explore a suitable CP-DFT approximation and discuss exact conditions, limitations, and results for selected examples.

==> tables/1d_ions.tex <==
\setlength{\tabcolsep}{12pt}

\begin{table*}[ht]
\centering
\renewcommand{\arraystretch}{2}
\begin{tabular}{ccccccc}
\hline
\hline
 $N_e$ &     Symbol & $V_{\ee}[n, \tilde n^{\text{BEA}}]$ & $V_{\ee}[n^{\text{LDA}}, \tilde n_{y}^{\text{BEA, LDA}}]$ & $V_{\ee}[n^{\text{LSDA}}, \tilde n_{x}^{\text{BEA, LSDA}}]$ & $V^{\text{HF}}_{\ee}$ &  $V^{\text{exact}}_{\ee}$ \\
\hline
     2 &         He &                      0.659 (-0.031) &                                     0.644 (-0.046) &                                     0.650 (-0.040) &         0.722 (0.032) &                     0.690 \\
     2 &     Li$^+$ &                      0.739 (-0.016) &                                     0.733 (-0.022) &                                     0.735 (-0.020) &         0.773 (0.018) &                     0.755 \\
     2 &  Be$^{++}$ &                      0.779 (-0.013) &                                     0.777 (-0.015) &                                     0.778 (-0.014) &         0.802 (0.010) &                     0.792 \\
     3 &         Li &                                   - &                                      1.855 (0.208) &                                      1.741 (0.094) &         1.682 (0.035) &                     1.647 \\
     3 &     Be$^+$ &                                   - &                                      2.069 (0.211) &                                      1.971 (0.113) &         1.881 (0.023) &                     1.858 \\
     4 &         Be &                                   - &                                      3.341 (0.153) &                                      3.314 (0.126) &         3.360 (0.172) &                     3.188 \\
\hline
\hline
\end{tabular}
\parbox{\textwidth}{\caption{
\unsure{reference in text. cleanup caption.}
\rp{Electron-electron repulsion energies, $V_{\ee}$, for 1D systems using various methods. In a pure CP-DFT approach we have $V^{\text{CP}}_{\ee}[n, \tilde n_y] = \half \int dy \, n(y) \int dy' \, \tilde n_y(y') \, v_{\text{exp}}(y - y')$ and the spin CP-DFT approach $V^{\text{CP}}_{\ee}[n, \tilde n_x] = \half \int dx \, n(x) \int dy' \, \tilde n_x(y') \, v_{\text{exp}}(y - y')$ . In the pure CP-DFT approach, unpolarized LDA is used in both the standard KS-DFT calculation (to obtain $n^{\text{LDA}}$) and the CP-KS calculations (to obtain $\tilde n_{y}^{\text{BEA, LDA}}$). In the spin CP-DFT approach, LSDA is used in both the standard KS-DFT calculation (to obtain $n^{\text{LSDA}}$) and the spin CP-KS calculations (to obtain $\tilde n_{x}^{\text{BEA, LSDA}}$). Errors with the exact are given in parenthesis. \label{tab: }}}}
\label{tab: bea ions}
\end{table*}
